Conditional Generative Modeling for Images, 3D Animations, and Video

This dissertation attempts to drive innovation in the field of generative modeling for computer vision, by exploring novel formulations of conditional generative models, and innovative applications in images, 3D animations, and video. Our research focuses on architectures that offer reversible transformations of noise and visual data, and the application of encoder-decoder architectures for generative tasks and 3D content manipulation. In all instances, we incorporate conditional information to enhance the synthesis of visual data, improving the efficiency of the generation process as well as the generated content. We introduce the use of Neural ODEs to model video dynamics using an encoder-decoder architecture, demonstrating their ability to predict future video frames despite being trained solely to reconstruct current frames. Next, we propose a conditional variant of continuous normalizing flows that enables higher-resolution image generation based on lower-resolution input, achieving comparable image quality while reducing parameters and training time. Our next contribution presents a pipeline that takes human images as input, automatically aligns a user-specified 3D character with the pose of the human, and facilitates pose editing based on partial inputs. Next, we derive the relevant mathematical details for denoising diffusion models that use non-isotropic Gaussian processes, and show comparable generation quality. Finally, we devise a novel denoising diffusion framework capable of solving all three video tasks of prediction, generation, and interpolation. We perform ablation studies, and show SOTA results on multiple datasets. Our contributions are published articles at peer-reviewed venues. Overall, our research aims to make a meaningful contribution to the pursuit of more efficient and flexible generative models, with the potential to shape the future of computer vision.

==> article1.tex <==
%% To change chapter header dynamically from french to english, use
%%\entetedynamique
\setcounter{corA}{0} % Pour recommancer à compter les def,
                     % theo, etc. à partir de 1
 % Pour écrire un article en français
\francais
 % Pour écrire un article en anglais
%%\anglais
%% NOTE: La plupart des macros ont un nom en anglais.
%% P.ex. \adresse et \address fonctionnent et sont équivalents.
%% \revue=\journal
%% \auteur=\author
%% \titre=\title

 % Nom de la revue de publication
\revue{Une revue}
\article{Titre de l'article}

 % Contribution(s) peronnelle(s) à l'article et rôle joué par tous les coauteurs
 %
 % Nécessaire seulement lorsque vous n'êtes pas seul·e auteur·e.
 % Les contributions peuvent apparaître ailleur dans la thèse.
 % Si \contributions est laissé vide (p.ex. si vous effacez
 % celui ci-bas), aucune contributions ne seront générées sur
 % la page titre de l'article.
 %
 % REMARQUE : L'exemple est sous forme d'\itemize,
 % mais toutes les constructions \LaTeX\ sont permises.
 % La commande peut aussi contenir un simple petit texte.
 %
 % La commande admet une option [<entête>]
\contributions%[Mes contributions et le rôle des coauteurs]
{
    \begin{itemize}
        \item Calcul de telle chose;
        \item Vérification de telle équation;
        \item Idée pour telle définition;
        \item Démonstration de tel théorème.
    \end{itemize}

    Le coauteur1 a suggéré telle chose.

    Le coauteur2 a fait telle calcul.\\[1cm]
}
%% Les contributions apparaîtrons après
%% \maketitle. Selon les goûts, il est
%% possible de mettre les contributions
%% avant, simplement en les écrivant
%% directement ici. Par exemple :
 % \section*{Contributions de <mon nom> et rôle joué par les coauteurs}
 % J'ai contribué en...
 %
 % Le rôle des coauteurs a été de...
 % \cleardoublepage

%%% INFORMATIONS POUR LA PAGE TITRE
 % Premier auteur·e et adresse
\auteur{Hima Ginère}
\adresse{1252i rue complexe\\ Université du plan complexe}
 % Deuxième auteur·e et adresse (si différente de la première)
%%\auteur{Hana Lietick}
%%\adresse{4242 rue imaginaire\\ Universität von der gau\ss sche Zahlenebene}
%%
%% et ainsi de suite pour les autres auteurs

\maketitle

\begin{resume}{Mots clés}
  Le résumé en français.
\end{resume}

\begin{abstract}{Key words}
  The english abstract.
\end{abstract}

\section{IntroductiPremieron}
%%
%% Le reste de l'article...
%%


Exemple de citation~: Consultez le \LaTeX\ companien
de Mittelbach {\it et al\/}\@. \cite{exemple}.

 % Pour générer la bibliographie à la fin
 % de l'article, utiliser la commande de la
 % classe <dms> \sectionbibliography{<nom du .bib>}.
 % Il y a aussi la possibilité d'utiliser le package
 % <chapterbib>, auquel cas on utilise simplement
 % \bibliography normalement.
 %
 % IMPORTANT : Dans tous les cas, il faut faire
 %    pdflatex these
 %    bibtex chapitre1
 %    bibtex chapitre2
 %    .
 %    .
 %    .
 %    bibtex chapitreN
 %    pdflatex these
 %    pdflatex these
 %
 % où <these> est le nom du .tex principal
 % (qui contient le \documentclass).
 % bibtex a besoin du .aux de chapitre1 et
 % non du .tex. Il est parfois nécessaire
 % d'effacer le .aux et de recommencer la
 % compilation du début.
%%\bibliographystyle{plain} % style plain anglais ou
\bibliographystyle{plain-fr} % style plain francais
%%\bibliographystyle{<style>} % autre
\sectionbibliography{ref.bib} %Donner le nom du .bib

\endinput
%%
%% End of file `article1.tex'.

